From Pixels to Prose: A Large Dataset of Dense Image Captions

Training large vision-language models requires extensive, high-quality image-text pairs. Existing web-scraped datasets, however, are noisy and lack detailed image descriptions. To bridge this gap, we introduce PixelProse, a comprehensive dataset of over 16M (million) synthetically generated captions, leveraging cutting-edge vision-language models for detailed and accurate descriptions. To ensure data integrity, we rigorously analyze our dataset for problematic content, including child sexual abuse material (CSAM), personally identifiable information (PII), and toxicity. We also provide valuable metadata such as watermark presence and aesthetic scores, aiding in further dataset filtering. We hope PixelProse will be a valuable resource for future vision-language research. PixelProse is available at https://huggingface.co/datasets/tomg-group-umd/pixelprose

==> tables/toxicity_scores.tex <==
\begin{table}[]
    \centering
    \caption{We assessed the distribution of various toxicity attributes in our captions. The attributes include toxicity, severe toxicity, obscenity, identity attacks, insults, threats, and sexually explicit content. The results indicate that the majority of captions fall within the lowest toxicity ranges (0-0.2). Comparatively, our VLM-generated captions exhibit a lower concentration of toxicity across all attributes, resulting in safer and more appropriate content.}
    \vspace{2mm}
    \scriptsize
    \setlength{\tabcolsep}{19pt} 
    \begin{tabular}{lccccc}
        \toprule
        Attribute            & 0-0.2 & 0.2-0.4 & 0.4-0.6 & 0.6-0.8 & 0.8-1.0 \\
        \midrule
        toxicity (original)            & 99.40 & 0.32 & 0.13 & 0.08 & 0.08 \\
        severe\_toxicity (original)     & 100.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        obscene (original)            & 99.96 & 0.02 & 0.01 & 0.01 & 0.01 \\
        identity\_attack (original)    & 99.93 & 0.05 & 0.01 & 0.00 & 0.00 \\
        insult (original)               & 99.73 & 0.13 & 0.06 & 0.04 & 0.04 \\
        threat (original)               & 99.96 & 0.02 & 0.01 & 0.01 & 0.00 \\
        sexual\_explicit (original)     & 99.98 & 0.01 & 0.00 & 0.00 & 0.00 \\
        \midrule
        toxicity (ours)         & 99.86 & 0.09 & 0.03 & 0.01 & 0.01 \\
        severe\_toxicity (ours) & 100.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        obscene (ours)          & 99.97 & 0.01 & 0.01 & 0.01 & 0.00 \\
        identity\_attack (ours) & 100.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        insult (ours)           & 99.93 & 0.05 & 0.01 & 0.00 & 0.00 \\
        threat (ours)           & 100.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        sexual\_explicit (ours) & 100.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        \bottomrule
    \end{tabular}
    \label{tab:toxicity_scores}
\end{table}

